Evolution of accretion disc reflection spectra due to a Type I X-ray burst

Irradiation of the accretion disc causes reflection signatures in the observed X-ray spectrum, encoding important information about the disc structure and density. A Type I X-ray burst will strongly irradiate the accretion disc and alter its properties. Previous numerical simulations predicted the evolution of the accretion disc due to an X-ray burst. Here, we process time-averaged simulation data of six time intervals to track changes in the reflection spectrum from the burst onset to just past its peak. We divide the reflecting region of the disc within $r\lesssim50$ km into 6-7 radial zones for every time interval and compute the reflection spectra for each zone. We integrate these reflection spectra to obtain a total reflection spectrum per time interval. The burst ionizes and heats the disc, which gradually weakens all emission lines. Compton scattering and bremsstrahlung rates increase in the disc during the burst rise, and the soft excess at $<$3 keV rises from $\approx4$% to $\approx38$% of the total emission at the burst peak. A soft excess is expected to be ubiquitous in the reflection spectra of X-ray bursts. Structural disc changes such as inflation because of heating or drainage of the inner disc due to Poynting-Robertson drag affect the strength of the soft excess. Further studies on the dependence of the reflection spectrum characteristics to changes in the accretion disc during an X-ray burst may lead to probes of the disc geometry.

==> references.tex <==
@article{ballantyne2002,
    author = {Ballantyne, D. R. and Ross, R. R.},
    title = "{The response of the Fe Kα line to changes in the X-ray illumination of accretion discs}",
    journal = {\mnras},
    volume = {332},
    number = {4},
    pages = {777-787},
    year = {2002},
    month = {06},
    abstract = "{X-ray reflection spectra from photoionized accretion discs in active galaxies are presented for a wide range of illumination conditions. The energy, equivalent width (EW) and flux of the Fe Kα line are shown to depend strongly on the ratio of illuminating flux to disc flux, Fx/Fdisc, the photon index of the irradiating power law, Γ, and the incidence angle of the radiation, i. When Fx/Fdisc≤2 a neutral Fe Kα line is prominent for all but the largest values of Γ. At higher illuminating fluxes an He-like Fe Kα line at 6.7 keV dominates the line complex. With a high-energy cut-off of 100 keV, the thermal ionization instability seems to suppress the ionized Fe Kα line when Γ≤1.6. The Fe Kα line flux correlates with Fx/Fdisc, but the dependence weakens as iron becomes fully ionized. The EW is roughly constant when Fx/Fdisc is low and a neutral line dominates, but then declines as the line progresses through higher ionization stages. There is a strong positive correlation between the Fe Kα EW and Γ when the line energy is at 6.7 keV, and a slight negative one when it is at 6.4 keV. This is a potential observational diagnostic of the ionization state of the disc. Observations of the broad Fe Kα line, which take into account any narrow component, would be able to test these predictions. Ionized Fe Kα lines at 6.7 keV are predicted to be common in a simple magnetic flare geometry. A model that includes multiple ionization gradients on the disc is postulated to reconcile the results with observations.}",
    issn = {0035-8711},
    doi = {10.1046/j.1365-8711.2002.05359.x},
    url = {https://doi.org/10.1046/j.1365-8711.2002.05359.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/332/4/777/5801287/332-4-777.pdf},
}


@article{fragile_2020, title={Interactions of type I X-ray bursts with thin accretion disks}, volume={4}, DOI={10.1038/s41550-019-0987-5}, number={5}, journal={Nature Astronomy}, author={Fragile, P. Chris and Ballantyne, David R. and Blankenship, Aidan}, year={2020}, pages={541–546}}

@ARTICLE{Eijnden2020,
       author = {{van den Eijnden}, J. and {Degenaar}, N. and {Ludlam}, R.~M. and {Parikh}, A.~S. and {Miller}, J.~M. and {Wijnands}, R. and {Gendreau}, K.~C. and {Arzoumanian}, Z. and {Chakrabarty}, D. and {Bult}, P.},
        title = "{A strongly changing accretion morphology during the outburst decay of the neutron star X-ray binary 4U 1608-52}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, stars: individual: (4U 1608-52), stars: neutron, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {493},
       number = {1},
        pages = {1318-1327},
          doi = {10.1093/mnras/staa423},
archivePrefix = {arXiv},
       eprint = {2002.04003},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.1318V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Fabian2000,
  author        = {{Fabian}, A.~C. and {Iwasawa}, K. and {Reynolds}, C.~S. and {Young}, A.~J.},
  journal       = {\pasp},
  title         = {{Broad Iron Lines in Active Galactic Nuclei}},
  year          = {2000},
  month         = sep,
  number        = {775},
  pages         = {1145-1161},
  volume        = {112},
  adsnote       = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl        = {https://ui.adsabs.harvard.edu/abs/2000PASP..112.1145F},
  archiveprefix = {arXiv},
  doi           = {10.1086/316610},
  eprint        = {astro-ph/0004366},
  keywords      = {accretion, accretion disks, black hole physics, Galaxies: Active, line: formation, line: profiles, X-rays: galaxies, Astrophysics},
  primaryclass  = {astro-ph},
}

@ARTICLE{Fabian1991,
       author = {{George}, I.~M. and {Fabian}, A.~C.},
        title = "{X-ray reflection from cold matter in Active Galactic Nuclei and X-ray binaries.}",
      journal = {\mnras},
     keywords = {Active Galactic Nuclei, Cold Plasmas, Computational Astrophysics, Dark Matter, X Ray Binaries, Abundance, Compton Effect, Fluorescence, Monte Carlo Method, X Ray Irradiation, Astrophysics},
         year = 1991,
        month = mar,
       volume = {249},
        pages = {352},
          doi = {10.1093/mnras/249.2.352},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991MNRAS.249..352G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ballantyne2004,
       author = {{Ballantyne}, D.~R.},
        title = "{Reflection spectra from an accretion disc illuminated by a neutron star X-ray burst}",
      journal = {\mnras},
     keywords = {Astrophysics},
         year = 2004,
        month = jun,
       volume = {351},
       number = {1},
        pages = {57-62},
          doi = {10.1111/j.1365-2966.2004.07767.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402603},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.351...57B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lightman1988,
       author = {{Lightman}, Alan P. and {White}, Timothy R.},
        title = "{Effects of Cold Matter in Active Galactic Nuclei: A Broad Hump in the X-Ray Spectra}",
      journal = {\apj},
     keywords = {Active Galactic Nuclei, Astronomical Spectroscopy, Dark Matter, Spectral Energy Distribution, X Ray Spectra, Black Holes (Astronomy), Optical Thickness, Spectrum Analysis, Astrophysics, GALAXIES: NUCLEI, X-RAYS: SPECTRA},
         year = 1988,
        month = dec,
       volume = {335},
        pages = {57},
          doi = {10.1086/166905},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...335...57L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2010,
       author = {{Garc{\'\i}a}, J. and {Kallman}, T.~R.},
        title = "{X-ray Reflected Spectra from Accretion Disk Models. I. Constant Density Atmospheres}",
      journal = {\apj},
     keywords = {accretion, accretion disks, atomic processes, black hole physics, line: formation, radiative transfer, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = aug,
       volume = {718},
       number = {2},
        pages = {695-706},
          doi = {10.1088/0004-637X/718/2/695},
archivePrefix = {arXiv},
       eprint = {1006.0485},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...718..695G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ross2005,
       author = {{Ross}, R.~R. and {Fabian}, A.~C.},
        title = "{A comprehensive range of X-ray ionized-reflection models}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, line: formation, radiative transfer, galaxies: active, X-rays: general, Astrophysics},
         year = 2005,
        month = mar,
       volume = {358},
       number = {1},
        pages = {211-216},
          doi = {10.1111/j.1365-2966.2005.08797.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0501116},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.358..211R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Nandra1994,
       author = {{Nandra}, K. and {Pounds}, K.~A.},
        title = "{GINGA observations of the X-ray spectra of Seyfert galaxies.}",
      journal = {\mnras},
         year = 1994,
        month = may,
       volume = {268},
        pages = {405-429},
          doi = {10.1093/mnras/268.2.405},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994MNRAS.268..405N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Szanecki2021,
       author = {{Szanecki}, Micha{\l} and {Nied{\'z}wiecki}, Andrzej and {Zdziarski}, Andrzej A.},
        title = "{Relativistic Reflection in NGC 4151}",
      journal = {\apj},
     keywords = {X-ray active galactic nuclei, Seyfert galaxies, Relativistic disks, Accretion, 2035, 1447, 1388, 14, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = mar,
       volume = {909},
       number = {2},
          eid = {205},
        pages = {205},
          doi = {10.3847/1538-4357/abe380},
archivePrefix = {arXiv},
       eprint = {2010.08358},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...909..205S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ballantyne2004apj,
       author = {{Ballantyne}, D.~R. and {Strohmayer}, T.~E.},
        title = "{The Evolution of the Accretion Disk around 4U 1820-30 during a Superburst}",
      journal = {\apjl},
     keywords = {Accretion, Accretion Disks, Line: Formation, Stars: Individual: Alphanumeric: 4U 1820-30, Stars: Neutron, X-Rays: Binaries, X-Rays: Bursts, Astrophysics},
         year = 2004,
        month = feb,
       volume = {602},
       number = {2},
        pages = {L105-L108},
          doi = {10.1086/382703},
archivePrefix = {arXiv},
       eprint = {astro-ph/0401154},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...602L.105B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maccarone2003,
       author = {{Maccarone}, T.~J. and {Coppi}, P.~S.},
        title = "{Spectral fits to the 1999 Aql X-1 outburst data}",
      journal = {\aap},
     keywords = {accretion, accretion disks, radiation mechanisms: non-thermal, X-rays: individual: Aql X-1, X-rays: bursts, Astrophysics},
         year = 2003,
        month = mar,
       volume = {399},
        pages = {1151-1157},
          doi = {10.1051/0004-6361:20021881},
archivePrefix = {arXiv},
       eprint = {astro-ph/0301091},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...399.1151M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Degenaar2013,
       author = {{Degenaar}, N. and {Miller}, J.~M. and {Wijnands}, R. and {Altamirano}, D. and {Fabian}, A.~C.},
        title = "{X-Ray Emission and Absorption Features during an Energetic Thermonuclear X-Ray Burst from IGR J17062-6143}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, stars: neutron, X-rays: binaries, X-rays: individual: IGR J17062{\textendash}6143, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = apr,
       volume = {767},
       number = {2},
          eid = {L37},
        pages = {L37},
          doi = {10.1088/2041-8205/767/2/L37},
archivePrefix = {arXiv},
       eprint = {1212.4869},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767L..37D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Cackett2008,
  author        = {{Cackett}, Edward M. and {Miller}, Jon M. and {Bhattacharyya}, Sudip and {Grindlay}, Jonathan E. and {Homan}, Jeroen and {van der Klis}, Michiel and {Miller}, M. Coleman and {Strohmayer}, Tod E. and {Wijnands}, Rudy},
  journal       = {\apj},
  title         = {{Relativistic Iron Emission Lines in Neutron Star Low-Mass X-Ray Binaries as Probes of Neutron Star Radii}},
  year          = {2008},
  month         = feb,
  number        = {1},
  pages         = {415-420},
  volume        = {674},
  adsnote       = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl        = {https://ui.adsabs.harvard.edu/abs/2008ApJ...674..415C},
  archiveprefix = {arXiv},
  doi           = {10.1086/524936},
  eprint        = {0708.3615},
  keywords      = {accretion, accretion disks, stars: neutron, X-rays: binaries, Astrophysics},
  primaryclass  = {astro-ph},
}

@ARTICLE{Xu2020,
       author = {{Xu}, Yanjun and {Harrison}, Fiona A. and {Tomsick}, John A. and {Hare}, Jeremy and {Fabian}, Andrew C. and {Walton}, Dominic J.},
        title = "{Evidence for Disk Truncation at Low Accretion States of the Black Hole Binary MAXI J1820+070 Observed by NuSTAR and XMM-Newton}",
      journal = {\apj},
     keywords = {14, 159, 1852, 1811, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = apr,
       volume = {893},
       number = {1},
          eid = {42},
        pages = {42},
          doi = {10.3847/1538-4357/ab7cdb},
archivePrefix = {arXiv},
       eprint = {2003.01778},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...893...42X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Popham2001,
       author = {{Popham}, Robert and {Sunyaev}, Rashid},
        title = "{Accretion Disk Boundary Layers around Neutron Stars: X-Ray Production in Low-Mass X-Ray Binaries}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Neutron, X-Rays: Stars, Astrophysics},
         year = 2001,
        month = jan,
       volume = {547},
       number = {1},
        pages = {355-383},
          doi = {10.1086/318336},
archivePrefix = {arXiv},
       eprint = {astro-ph/0004017},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...547..355P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ding2021,
       author = {{Ding}, G.~Q. and {Chen}, T.~T. and {Qu}, J.~L.},
        title = "{A study of the hard X-ray spectral tails in Scorpius X-1 using RXTE observations}",
      journal = {\mnras},
     keywords = {stars: neutron, X-rays: binaries, X-rays: individual: Scorpius X-1, X-rays: stars},
         year = 2021,
        month = jan,
       volume = {500},
       number = {1},
        pages = {772-785},
          doi = {10.1093/mnras/staa2990},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500..772D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Galeev1979,
       author = {{Galeev}, A.~A. and {Rosner}, R. and {Vaiana}, G.~S.},
        title = "{Structured coronae of accretion disks.}",
      journal = {\apj},
     keywords = {Binary Stars, Coronas, Cosmic X Rays, Magnetohydrodynamics, Stellar Mass Accretion, X Ray Sources, Buoyancy, Convection Currents, Cooling, Energy Dissipation, Interstellar Gas, Interstellar Magnetic Fields, Stellar Luminosity, Thermal Plasmas, Astrophysics, Accretion Disks:Magnetic Fields, Accretion Disks:Magnetohydrodynamics, Accretion Disks:Stellar Coronae, Accretion Disks:X-Ray Binaries, Accretion Disks:X-Ray Sources},
         year = 1979,
        month = apr,
       volume = {229},
        pages = {318-326},
          doi = {10.1086/156957},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...229..318G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ross1993,
       author = {{Ross}, R.~R. and {Fabian}, A.~C.},
        title = "{The effects of photoionization on X-ray reflection spectra in active galactic nuclei.}",
      journal = {\mnras},
     keywords = {Accretion Disks, Active Galactic Nuclei, Black Holes (Astronomy), Computational Astrophysics, Photoionization, X Ray Spectra, Fluorescence, Iron, Stellar Mass Accretion, X Ray Absorption, X Ray Scattering, Astrophysics},
         year = 1993,
        month = mar,
       volume = {261},
        pages = {74-82},
          doi = {10.1093/mnras/261.1.74},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993MNRAS.261...74R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garcia2020,
       author = {{Garc{\'\i}a}, Javier A. and {Sokolova-Lapa}, Ekaterina and {Dauser}, Thomas and {Madej}, Jerzy and {R{\'o}{\.z}a{\'n}ska}, Agata and {Majczyna}, Agnieszka and {Harrison}, Fiona A. and {Wilms}, J{\"o}rn},
        title = "{Accurate Treatment of Comptonization in X-Ray Illuminated Accretion Disks}",
      journal = {\apj},
     keywords = {1967, 1857, 1579, 14, 159, 2099, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jul,
       volume = {897},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ab919b},
archivePrefix = {arXiv},
       eprint = {2005.04852},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...897...67G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Garcia2011,
       author = {{Garc{\'\i}a}, J. and {Kallman}, T.~R. and {Mushotzky}, R.~F.},
        title = "{X-ray Reflected Spectra from Accretion Disk Models. II. Diagnostic Tools for X-ray Observations}",
      journal = {\apj},
     keywords = {accretion, accretion disks, atomic processes, black hole physics, line: formation, radiative transfer, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = apr,
       volume = {731},
       number = {2},
          eid = {131},
        pages = {131},
          doi = {10.1088/0004-637X/731/2/131},
archivePrefix = {arXiv},
       eprint = {1101.1115},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...731..131G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Degenaar2018,
       author = {{Degenaar}, Nathalie and {Ballantyne}, David R. and {Belloni}, Tomaso and {Chakraborty}, Manoneeta and {Chen}, Yu-Peng and {Ji}, Long and {Kretschmar}, Peter and {Kuulkers}, Erik and {Li}, Jian and {Maccarone}, Thomas J. and {Malzac}, Julien and {Zhang}, Shu and {Zhang}, Shuang-Nan},
        title = "{Accretion Disks and Coronae in the X-Ray Flashlight}",
      journal = {\ssr},
     keywords = {Accretion, accretion disks, Stars: coronae, Stars: jets, Stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = feb,
       volume = {214},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.1007/s11214-017-0448-3},
archivePrefix = {arXiv},
       eprint = {1711.06272},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018SSRv..214...15D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lewin1993,
       author = {{Lewin}, Walter H.~G. and {van Paradijs}, Jan and {Taam}, Ronald E.},
        title = "{X-Ray Bursts}",
      journal = {\ssr},
         year = 1993,
        month = sep,
       volume = {62},
       number = {3-4},
        pages = {223-389},
          doi = {10.1007/BF00196124},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993SSRv...62..223L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{leblanc_2010, place={Chichester}, title={An introduction to stellar astrophysics}, publisher={Wiley}, author={LeBlanc, Francis}, year={2010}}



@ARTICLE{Koliopanos2021,
       author = {{Koliopanos}, Filippos and {Vasilopoulos}, Georgios and {Guillot}, Sebastien and {Webb}, Natalie},
        title = "{Disappearance of the Fe K {\ensuremath{\alpha}} emission line in ultracompact X-ray binaries 4U 1543-624 and Swift J1756.9-2508}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, line: formation, radiative transfer, methods: observational, techniques: spectroscopic, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jan,
       volume = {500},
       number = {4},
        pages = {5603-5613},
          doi = {10.1093/mnras/staa3490},
archivePrefix = {arXiv},
       eprint = {2001.00713},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.5603K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keek2018,
       author = {{Keek}, L. and {Arzoumanian}, Z. and {Bult}, P. and {Cackett}, E.~M. and {Chakrabarty}, D. and {Chenevez}, J. and {Fabian}, A.~C. and {Gendreau}, K.~C. and {Guillot}, S. and {G{\"u}ver}, T. and {Homan}, J. and {Jaisawal}, G.~K. and {Lamb}, F.~K. and {Ludlam}, R.~M. and {Mahmoodifar}, S. and {Markwardt}, C.~B. and {Miller}, J.~M. and {Prigozhin}, G. and {Soong}, Y. and {Strohmayer}, T.~E. and {Wolff}, M.~T.},
        title = "{NICER Observes the Effects of an X-Ray Burst on the Accretion Environment in Aql X-1}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, stars: individual: Aql X-1, stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = mar,
       volume = {855},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.3847/2041-8213/aab104},
archivePrefix = {arXiv},
       eprint = {1808.06441},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...855L...4K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keek2017,
       author = {{Keek}, L. and {Iwakiri}, W. and {Serino}, M. and {Ballantyne}, D.~R. and {in't Zand}, J.~J.~M. and {Strohmayer}, T.~E.},
        title = "{X-Ray Reflection and an Exceptionally Long Thermonuclear Helium Burst from IGR J17062-6143}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: individual: IGR J17062-6143, stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = feb,
       volume = {836},
       number = {1},
          eid = {111},
        pages = {111},
          doi = {10.3847/1538-4357/836/1/111},
archivePrefix = {arXiv},
       eprint = {1610.07608},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...836..111K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zand2013,
       author = {{in't Zand}, J.~J.~M. and {Galloway}, D.~K. and {Marshall}, H.~L. and {Ballantyne}, D.~R. and {Jonker}, P.~G. and {Paerels}, F.~B.~S. and {Palmer}, D.~M. and {Patruno}, A. and {Weinberg}, N.~N.},
        title = "{A bright thermonuclear X-ray burst simultaneously observed with Chandra and RXTE}",
      journal = {\aap},
     keywords = {accretion, accretion disks, X-rays: binaries, X-rays: bursts, stars: neutron, X-rays: individuals: SAX J1808.4-3658, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = may,
       volume = {553},
          eid = {A83},
        pages = {A83},
          doi = {10.1051/0004-6361/201321056},
archivePrefix = {arXiv},
       eprint = {1301.2232},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...553A..83I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bult2019,
       author = {{Bult}, Peter and {Jaisawal}, Gaurava K. and {G{\"u}ver}, Tolga and {Strohmayer}, Tod E. and {Altamirano}, Diego and {Arzoumanian}, Zaven and {Ballantyne}, David R. and {Chakrabarty}, Deepto and {Chenevez}, J{\'e}r{\^o}me and {Gendreau}, Keith C. and {Guillot}, Sebastien and {Ludlam}, Renee M.},
        title = "{A NICER Thermonuclear Burst from the Millisecond X-Ray Pulsar SAX J1808.4-3658}",
      journal = {\apjl},
     keywords = {X-ray bursts, Millisecond pulsars, 1814, 1062, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = nov,
       volume = {885},
       number = {1},
          eid = {L1},
        pages = {L1},
          doi = {10.3847/2041-8213/ab4ae1},
archivePrefix = {arXiv},
       eprint = {1909.03595},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...885L...1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chen2019,
       author = {{Chen}, Y.~P. and {Zhang}, S. and {Zhang}, S.~N. and {Ji}, L. and {Kong}, L.~D. and {Santangelo}, A. and {Qu}, J.~L. and {Lu}, F.~J. and {Li}, T.~P. and {Song}, L.~M. and {Xu}, Y.~P. and {Cao}, X.~L. and {Chen}, Y. and {Liu}, C.~Z. and {Bu}, Q.~C. and {Cai}, C. and {Chang}, Z. and {Chen}, G. and {Chen}, L. and {Chen}, T.~X. and {Chen}, Y.~B. and {Cui}, W. and {Cui}, W.~W. and {Deng}, J.~K. and {Dong}, Y.~W. and {Du}, Y.~Y. and {Fu}, M.~X. and {Gao}, G.~H. and {Gao}, H. and {Gao}, M. and {Ge}, M.~Y. and {Gu}, Y.~D. and {Guan}, J. and {Guo}, C.~C. and {Han}, D.~W. and {Huang}, Y. and {Huo}, J. and {Jia}, S.~M. and {Jiang}, L.~H. and {Jiang}, W.~C. and {Jin}, J. and {Li}, B. and {Li}, C.~K. and {Li}, G. and {Li}, M.~S. and {Li}, W. and {Li}, X. and {Li}, X.~B. and {Li}, X.~F. and {Li}, Y.~G. and {Li}, Z.~W. and {Liang}, X.~H. and {Liao}, J.~Y. and {Liu}, G.~Q. and {Liu}, H.~W. and {Liu}, X.~J. and {Liu}, Y.~N. and {Lu}, B. and {Lu}, X.~F. and {Luo}, Q. and {Luo}, T. and {Ma}, X. and {Meng}, B. and {Nang}, Y. and {Nie}, J.~Y. and {Ou}, G. and {Ren}, X.~Q. and {Sai}, N. and {Sun}, L. and {Tan}, Y. and {Tao}, L. and {Tuo}, Y.~L. and {Wang}, C. and {Wang}, G.~F. and {Wang}, J. and {Wang}, W.~S. and {Wang}, Y.~S. and {Wen}, X.~Y. and {Wu}, B.~Y. and {Wu}, B.~B. and {Wu}, M. and {Xiao}, G.~C. and {Xiao}, S. and {Xiong}, S.~L. and {Yang}, J.~W. and {Yang}, S. and {Yang}, Y.~J. and {Yang}, Y.~J. and {Yi}, Q.~B. and {Yin}, Q.~Q. and {You}, Y. and {Zhang}, A.~M. and {Zhang}, C.~L. and {Zhang}, C.~M. and {Zhang}, F. and {Zhang}, H.~M. and {Zhang}, J. and {Zhang}, T. and {Zhang}, W.~C. and {Zhang}, W. and {Zhang}, W.~Z. and {Zhang}, Yi. and {Zhang}, Y.~F. and {Zhang}, Y.~J. and {Zhang}, Y. and {Zhang}, Z. and {Zhang}, Z.~L. and {Zhao}, H.~S. and {Zhao}, X.~F. and {Zheng}, S.~J. and {Zhou}, D.~K. and {Zhou}, J.~F. and {Zhu}, Y. and {Zhu}, Y.~X.},
        title = "{Insight-HXMT observation on 4U 1608-52: Evolving spectral properties of a bright type-I X-ray burst}",
      journal = {Journal of High Energy Astrophysics},
     keywords = {Stars: coronae, Stars: neutron, X-rays: individual (4U 1608-52), X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = nov,
       volume = {24},
        pages = {23-29},
          doi = {10.1016/j.jheap.2019.09.001},
archivePrefix = {arXiv},
       eprint = {1910.08220},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019JHEAp..24...23C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Worpel2013,
       author = {{Worpel}, Hauke and {Galloway}, Duncan K. and {Price}, Daniel J.},
        title = "{Evidence for Accretion Rate Change during Type I X-Ray Bursts}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: neutron, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = aug,
       volume = {772},
       number = {2},
          eid = {94},
        pages = {94},
          doi = {10.1088/0004-637X/772/2/94},
archivePrefix = {arXiv},
       eprint = {1303.4824},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...772...94W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miller2007,
       author = {{Miller}, J.~M.},
        title = "{Relativistic X-Ray Lines from the Inner Accretion Disks Around Black Holes}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = 2007,
        month = sep,
       volume = {45},
       number = {1},
        pages = {441-479},
          doi = {10.1146/annurev.astro.45.051806.110555},
archivePrefix = {arXiv},
       eprint = {0705.0540},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ARA&A..45..441M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fernandez2020,
       author = {{S{\'a}nchez-Fern{\'a}ndez}, C. and {Kajava}, J.~J.~E. and {Poutanen}, J. and {Kuulkers}, E. and {Suleimanov}, V.~F.},
        title = "{Burst-induced coronal cooling in GS 1826-24. The clock wagging its tail}",
      journal = {\aap},
     keywords = {stars: neutron, dense matter, accretion, accretion disks, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {634},
          eid = {A58},
        pages = {A58},
          doi = {10.1051/0004-6361/201936599},
archivePrefix = {arXiv},
       eprint = {2002.03654},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...634A..58S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Speicher2020,
       author = {{Speicher}, J. and {Ballantyne}, D.~R. and {Malzac}, J.},
        title = "{Cooling of accretion disc coronae by Type I X-ray bursts}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, radiation mechanisms: thermal, stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {499},
       number = {3},
        pages = {4479-4489},
          doi = {10.1093/mnras/staa3137},
archivePrefix = {arXiv},
       eprint = {2010.05791},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.499.4479S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ballantyne2002code,
       author = {{Ballantyne}, D.~R. and {Ross}, R.~R. and {Fabian}, A.~C.},
        title = "{Soft X-ray emission lines from photoionized accretion discs: constraints on their strength and width}",
      journal = {\mnras},
     keywords = {line: formation, radiative transfer, galaxies: active, galaxies: individual: MCG-6-30-15, X-rays: galaxies, X-rays: general, Astrophysics},
         year = 2002,
        month = nov,
       volume = {336},
       number = {3},
        pages = {867-872},
          doi = {10.1046/j.1365-8711.2002.05818.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0202148},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.336..867B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ballantyne2001,
       author = {{Ballantyne}, D.~R. and {Ross}, R.~R. and {Fabian}, A.~C.},
        title = "{X-ray reflection by photoionized accretion discs}",
      journal = {\mnras},
     keywords = {ACCRETION, ACCRETION DISCS, LINE: PROFILES, RADIATIVE TRANSFER, GALAXIES: ACTIVE, X-RAYS: GENERAL, Astrophysics},
         year = 2001,
        month = oct,
       volume = {327},
       number = {1},
        pages = {10-22},
          doi = {10.1046/j.1365-8711.2001.04432.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0102040},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.327...10B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Galloway2021,
       author = {{Galloway}, Duncan K. and {Keek}, Laurens},
        title = "{Thermonuclear X-ray Bursts}",
      journal = {Astrophysics and Space Science Library},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = jan,
       volume = {461},
        pages = {209-262},
          doi = {10.1007/978-3-662-62110-3\_5},
archivePrefix = {arXiv},
       eprint = {1712.06227},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ASSL..461..209G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Norris2005,
       author = {{Norris}, J.~P. and {Bonnell}, J.~T. and {Kazanas}, D. and {Scargle}, J.~D. and {Hakkila}, J. and {Giblin}, T.~W.},
        title = "{Long-Lag, Wide-Pulse Gamma-Ray Bursts}",
      journal = {\apj},
     keywords = {Gamma Rays: Bursts, ISM: Jets and Outflows, Astrophysics},
         year = 2005,
        month = jul,
       volume = {627},
       number = {1},
        pages = {324-345},
          doi = {10.1086/430294},
archivePrefix = {arXiv},
       eprint = {astro-ph/0503383},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...627..324N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Strohmayer2002,
       author = {{Strohmayer}, Tod E. and {Brown}, Edward F.},
        title = "{A Remarkable 3 Hour Thermonuclear Burst from 4U 1820-30}",
      journal = {\apj},
     keywords = {Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Individual: Alphanumeric: 4U 1820-30, Stars: Neutron, X-Rays: Binaries, X-Rays: Bursts, Astrophysics},
         year = 2002,
        month = feb,
       volume = {566},
       number = {2},
        pages = {1045-1059},
          doi = {10.1086/338337},
archivePrefix = {arXiv},
       eprint = {astro-ph/0108420},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...566.1045S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keek2014,
       author = {{Keek}, L. and {Ballantyne}, D.~R. and {Kuulkers}, E. and {Strohmayer}, T.~E.},
        title = "{Characterizing the Evolving X-Ray Spectral Features during a Superburst from 4U 1636-536}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: individual: 4U 1636{\textendash}536, stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = jul,
       volume = {789},
       number = {2},
          eid = {121},
        pages = {121},
          doi = {10.1088/0004-637X/789/2/121},
archivePrefix = {arXiv},
       eprint = {1403.4940},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...789..121K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gendreau2017,
       author = {{Gendreau}, Keith and {Arzoumanian}, Zaven},
        title = "{Searching for a pulse}",
      journal = {Nature Astronomy},
         year = 2017,
        month = dec,
       volume = {1},
        pages = {895-895},
          doi = {10.1038/s41550-017-0301-3},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017NatAs...1..895G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keek2014ApJL,
       author = {{Keek}, L. and {Ballantyne}, D.~R. and {Kuulkers}, E. and {Strohmayer}, T.~E.},
        title = "{X-Raying an Accretion Disk in Realtime: The Evolution of Ionized Reflection during a Superburst from 4U 1636-536}",
      journal = {\apjl},
     keywords = {accretion, accretion disks, stars: individual: 4U 1636-536, stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = dec,
       volume = {797},
       number = {2},
          eid = {L23},
        pages = {L23},
          doi = {10.1088/2041-8205/797/2/L23},
archivePrefix = {arXiv},
       eprint = {1410.5434},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...797L..23K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Keek2016,
       author = {{Keek}, L. and {Wolf}, Z. and {Ballantyne}, D.~R.},
        title = "{Accretion Disk Signatures in Type I X-Ray Bursts: Prospects for Future Missions}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: neutron, X-rays: binaries, X-rays: bursts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = jul,
       volume = {826},
       number = {1},
          eid = {79},
        pages = {79},
          doi = {10.3847/0004-637X/826/1/79},
archivePrefix = {arXiv},
       eprint = {1605.06113},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826...79K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Walker1992,
       author = {{Walker}, Mark A.},
        title = "{Radiation Dynamics in X-Ray Binaries. I. Type 1 Bursts}",
      journal = {\apj},
     keywords = {Accretion Disks, Neutron Stars, Stellar Radiation, X Ray Binaries, Computational Astrophysics, Thermonuclear Reactions, Astrophysics, ACCRETION, ACCRETION DISKS, RADIATION MECHANISMS: THERMAL, STARS: NEUTRON, X-RAYS: BURSTS},
         year = 1992,
        month = feb,
       volume = {385},
        pages = {642},
          doi = {10.1086/170969},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992ApJ...385..642W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Worpel2015,
       author = {{Worpel}, Hauke and {Galloway}, Duncan K. and {Price}, Daniel J.},
        title = "{Evidence for Enhanced Persistent Emission During Sub-Eddington Thermonuclear Bursts}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: neutron, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = mar,
       volume = {801},
       number = {1},
          eid = {60},
        pages = {60},
          doi = {10.1088/0004-637X/801/1/60},
archivePrefix = {arXiv},
       eprint = {1501.02070},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...801...60W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cackett2010,
       author = {{Cackett}, Edward M. and {Miller}, Jon M. and {Ballantyne}, David R. and {Barret}, Didier and {Bhattacharyya}, Sudip and {Boutelier}, Martin and {Miller}, M. Coleman and {Strohmayer}, Tod E. and {Wijnands}, Rudy},
        title = "{Relativistic Lines and Reflection from the Inner Accretion Disks Around Neutron Stars}",
      journal = {\apj},
     keywords = {accretion, accretion disks, stars: neutron, X-rays: binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = sep,
       volume = {720},
       number = {1},
        pages = {205-225},
          doi = {10.1088/0004-637X/720/1/205},
archivePrefix = {arXiv},
       eprint = {0908.1098},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...720..205C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ross1978,
       author = {{Ross}, R.~R. and {Weaver}, R. and {McCray}, R.},
        title = "{The Comptonization of iron X-ray features in compact X-ray sources.}",
      journal = {\apj},
     keywords = {Compton Effect, Iron, Radiative Transfer, X Ray Sources, X Ray Spectra, Emission Spectra, Fokker-Planck Equation, Photoionization, Stellar Models, Astrophysics, Spectra:X-Ray Sources, X-Ray Sources: Compton Scattering},
         year = 1978,
        month = jan,
       volume = {219},
        pages = {292-299},
          doi = {10.1086/155776},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978ApJ...219..292R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Suleimanov2011,
       author = {{Suleimanov}, V. and {Poutanen}, J. and {Werner}, K.},
        title = "{X-ray bursting neutron star atmosphere models: spectra and color corrections}",
      journal = {\aap},
     keywords = {radiative transfer, scattering, methods: numerical, stars: neutron, stars: atmospheres, X-rays: stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = mar,
       volume = {527},
          eid = {A139},
        pages = {A139},
          doi = {10.1051/0004-6361/201015845},
archivePrefix = {arXiv},
       eprint = {1009.6147},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...527A.139S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Suleimanov2012,
       author = {{Suleimanov}, V. and {Poutanen}, J. and {Werner}, K.},
        title = "{X-ray bursting neutron star atmosphere models using an exact relativistic kinetic equation for Compton scattering}",
      journal = {\aap},
     keywords = {radiative transfer, scattering, methods: numerical, stars: atmospheres, stars: neutron, X-rays: stars, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = sep,
       volume = {545},
          eid = {A120},
        pages = {A120},
          doi = {10.1051/0004-6361/201219480},
archivePrefix = {arXiv},
       eprint = {1208.1467},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...545A.120S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Rybicki1986,
       author = {{Rybicki}, George B. and {Lightman}, Alan P.},
        title = "{Radiative Processes in Astrophysics}",
         year = 1986,
         publisher = "{Wiley}",
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986rpa..book.....R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Inogamov2010,
       author = {{Inogamov}, N.~A. and {Sunyaev}, R.~A.},
        title = "{Spread of matter over a neutron-star surface during disk accretion: Deceleration of rapid rotation}",
      journal = {Astronomy Letters},
     keywords = {disk accretion, neutron stars, boundary layer, X-ray sources, X-ray bursters, low-mass X-ray binaries, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = dec,
       volume = {36},
       number = {12},
        pages = {848-894},
          doi = {10.1134/S1063773710120029},
archivePrefix = {arXiv},
       eprint = {1102.0975},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AstL...36..848I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Inogamov1999,
       author = {{Inogamov}, N.~A. and {Sunyaev}, R.~A.},
        title = "{Spread of matter over a neutron-star surface during disk accretion}",
      journal = {Astronomy Letters},
     keywords = {Astrophysics},
         year = 1999,
        month = may,
       volume = {25},
       number = {5},
        pages = {269-293},
archivePrefix = {arXiv},
       eprint = {astro-ph/9904333},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999AstL...25..269I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ross1979,
       author = {{Ross}, R.~R.},
        title = "{Spectral formation in compact X-ray sources.}",
      journal = {\apj},
     keywords = {Cosmic X Rays, Galactic Radiation, Radiative Transfer, Spectrum Analysis, X Ray Sources, X Ray Spectra, Astronomical Models, Compton Effect, Continuous Radiation, Fokker-Planck Equation, Gas Temperature, Ionized Gases, Optical Thickness, Photoabsorption, Point Sources, Thomson Scattering, X Ray Scattering, Astrophysics, Line Formation:X-Ray Sources, Radiative Transfer:X Rays, X-Ray Sources:Models},
         year = 1979,
        month = oct,
       volume = {233},
        pages = {334-343},
          doi = {10.1086/157394},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...233..334R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hoffman1977,
       author = {{Hoffman}, J.~A. and {Lewin}, W.~H.~G. and {Doty}, J.},
        title = "{Observations of the X-ray burst source MXB 1636-53.}",
      journal = {\apjl},
     keywords = {Sas, Spaceborne Astronomy, X Ray Sources, Emission Spectra, Radiation Distribution, Astronomy},
         year = 1977,
        month = oct,
       volume = {217},
        pages = {L23-L28},
          doi = {10.1086/182531},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977ApJ...217L..23H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


